Overcoming Blind Spots: Occlusion Considerations for Improved Autonomous Driving Safety

Our work introduces a module for assessing the trajectory safety of autonomous vehicles in dynamic environments marked by high uncertainty. We focus on occluded areas and occluded traffic participants with limited information about surrounding obstacles. To address this problem, we propose a software module that handles blind spots (BS) created by static and dynamic obstacles in urban environments. We identify potential occluded traffic participants, predict their movement, and assess the ego vehicle's trajectory using various criticality metrics. The method offers a straightforward and modular integration into motion planner algorithms. We present critical real-world scenarios to evaluate our module and apply our approach to a publicly available trajectory planning algorithm. Our results demonstrate that safe yet efficient driving with occluded road users can be achieved by incorporating safety assessments into the planning process. The code used in this research is publicly available as open-source software and can be accessed at the following link: https://github.com/TUM-AVS/Frenetix-Occlusion.

==> chapters/99_archive.tex <==
\begin{algorithm}[!ht]
\caption{Determine Spawn Points for PA}
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\SetKw{KwBy}{by}
\SetKwFunction{FMain}{Main}
\SetKwFunction{FSub}{Sub}
\SetKwProg{Fn}{Function}{:}{}

\Input{$\mathbf{p}_{\text{ego}}, \theta_{\text{ego}}, \mathbf{c}_{\text{ego}}, v_{\text{ego}}$}
\Output{List of potential SpawnPoint objects $\mathcal{S}$}
\BlankLine


$\mathcal{S} \leftarrow \{\}$ \tcp*{Initialize spawn points list}
$\mathbf{p}_{\text{ego}}, \theta_{\text{ego}}, \mathbf{c}_{\text{ego}} \leftarrow$ Update with current state \;
$\Gamma_\mathrm{s} \leftarrow$ Prepare reference path ($\Gamma$)\;
$\iota \leftarrow$ Determine ego intention ($\Gamma_\mathrm{s}$)\;

\If{dynamic and ($\iota =$ 'left' or $\iota =$ 'right')}{
    $\mathcal{S}_{\text{turn}} \leftarrow$ Find spawn point behind turn($\iota$)\;
    Append $\mathcal{S}_{\text{turn}}$ to $\mathcal{S}$\;
}
\If{static}{
    \If{$\iota =$ 'straight' or $\iota =$ 'left'}{
        $\mathcal{S}_{\text{dyn}} \leftarrow$ Find spawn point behind dynamic obstacle()\;
        Append $\mathcal{S}_{\text{dyn}}$ to $\mathcal{S}$\;
    }
    \If{static}{
        $\mathcal{S}_{\text{stat}} \leftarrow$ Find spawn point behind static obstacle()\;
        Append $\mathcal{S}_{\text{stat}}$ to $\mathcal{S}$\;
    }
}
\Return{$\mathcal{S}$}\;
\end{algorithm}
